Diversity Curves for Graph Representation Learning

Graph-level representations are crucial tools for characterising structural differences between graphs. However, comparing graphs with different cardinalities, even when sampled from the same underlying distribution, remains challenging. Unsupervised tasks in particular require interpretable, scalable, and reliable size-aware graph representations. Our work addresses these issues by tracking the structural diversity of a graph across coarsening levels. The resulting graph embeddings, which we denote diversity curves, are interpretable by construction, efficient, and directly comparable across coarsening hierarchies. Specifically, we track the spread of graphs, a novel isometry invariant that is inherently well-suited for encoding the metric diversity and geometry of graphs. We utilise edge contraction coarsening and prove that this improves expressivity, thus leading to more powerful graph-level representations than structural descriptors alone. Demonstrating their utility over a range of baseline methods in practice, we use diversity curves to (i) cluster and visualise simulated graphs across varying sizes, (ii) distinguish the geometry of single-cell graphs, (iii) compare the structure of molecular graph datasets, and (iv) characterise geometric shapes.

==> tables/expressivity_main.tex <==
% \begin{table}[ht]

% \caption{Number of pairs from the \texttt{BREC} dataset distinguished via structural diversity or diversity curves. Compared to representative results from \citep{wang2023empirical,southern2023curvature, ballester2025expressivity}.}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llccccc}
% \toprule
%  Method & Details & Basic (60) & Regular (140) & Extension (100) & CFI (100) & All (400) \\
% \midrule
% %1 WL (from \citep{southern2023curvature})  & 56 (93.3\%)  & 50 (50.0\%) & 97 (97.0\%)  & 4 (4.0\%) & 207 (51.8\%)\\
% %3 WL (from \citep{southern2023curvature})  & 56 (93.3\%)  & 50 (50.0\%) & 100 (97.0\%)  & 59 (4.0\%) &  (51.8\%)\\
% %\midrule
% %Resistance Curvature (from \citep{southern2023curvature})  & 56 (93.3\%)  & 50 (50.0\%) & 97 (97.0\%)  & 4 (4.0\%) & 207 (51.8\%)\\
% %OR Curvature (from \citep{southern2023curvature})  & 56 (93.3\%)  & 50 (50.0\%) & 97 (97.0\%)  & 4 (4.0\%) & 207 (51.8\%)\\
% 3 WL &(from \citep{wang2023empirical})  & 60 (100.0\%)  & 50 (35.7\%) & 100 (100.0\%)  & 60 (60.0\%) & 270 (67.5\%)\\
% 1 WL &(from \citep{southern2023curvature})  & 0 (0.0\%)  & 0 (0.0\%) & 0 (0.0\%)  & 0 (0.0\%) & 0 (0.0\%)\\
% \midrule
% % I2-GNN &(from \citep{wang2023empirical})  & 60 (100.0\%)  & 100 (71.4\%) & 100 (100.0\%)  & 0 (0.0\%) & 281 (70.2\%)\\
% % KP-GNN &(from \citep{wang2023empirical})  & 60 (100.0\%)  & 106 (75.7\%) & 98 (98.0\%)  & 11 (11.0\%) & 275 (68.8\%)\\
% % GSN &(from \citep{wang2023empirical})  & 60 (100.0\%)  & 99 (70.7\%) & 95 (95.0\%)  & 0 (0.0\%) & 254 (63.5\%)\\
% % Graphormer &(from \citep{wang2023empirical})  & 16 (26.7\%)  & 12 (8.6\%) & 41 (41.0\%)  & 10 (10.0\%) & 79 (19.8\%)\\
% % \midrule
% % CurvPool &(from \citep{lachi2025expressive})  & 35 (58.3\%)  & 65 (46.4.0\%) & 53 (53.0\%)  & 4 (4.0\%) & 157 (39.3\%)\\
% % XP &(from \citep{lachi2025expressive})  & 48 (80.0\%)  & 3 (0.02\%) & 72 (72.0\%)  & 1 (1.0\%) & 124 (31.0\%)\\
% % EdgePool &(from \citep{lachi2025expressive})  & 13 (21.7\%)  & 0 (0.0\%) & 10 (0.1\%)  & 0 (0.0\%) & 23 (5.8\%)\\
% % DiffPool &(from \citep{lachi2025expressive})  & 0 (0.0\%)  & 0 (0.0\%) & 0 (0.0\%)  & 0 (0.0\%) & 0 (0.0\%)\\
% % \midrule
% % PH Laplacian & (from \citep{ballester2025expressivity}) & 60 (100\%) & 74 (53\%) & 100 (100\%) &6 (6\%) & 216 (54\%) \\
% % PH Ollivier–Ricci Curvature & (from \citep{ballester2025expressivity}) & 60 (100\%) & 76 (54\%) & 92 (92\%) & 3 (3\%) & 208 (52\%) \\
% % PH Forman–Ricci Curvature & (from \citep{ballester2025expressivity}) & 59 (98\%) & 70 (50\%) & 59 (59\%) & 3 (3\%) & 172 (43\%) \\
% % PH Degree Filtration & (from \citep{ballester2025expressivity}) & 47 (78\%) & 55 (39\%) & 26 (26\%) & 3 (3\%) & 116 (29\%) \\
% PH Vietoris-Rips & (from \citep{ballester2025expressivity}) & 31 (52\%) & 55 (39\%) & 11 (11\%) & 3 (3\%) & 84 (21\%) \\
% %\midrule
% %PH1 Laplacian & (from \citep{ballester2025expressivity}) & 60 (100\%) & 1 (1\%) & 94 (94\%) & 6 (6\%) & 160 (40\%) \\
% %PH1 Ollivier–Ricci Curvature & (from \citep{ballester2025expressivity}) & 56 (93\%) & 59 (42\%)  & 76 (76\%)  & 3 (3\%)    & 176 (44\%) \\
% %PH1 Forman–Ricci Curvature & (from \citep{ballester2025expressivity}) & 52 (87\%) & 45 (32\%)  & 44 (44\%)  & 3 (3\%)    & 132 (33\%) \\
% %PH1 Degree Filtration & (from \citep{ballester2025expressivity}) & 2 (3\%)   & 0 (0\%)    & 7 (7\%)    & 3 (3\%)    & 12 (3\%)   \\
% %PH1 Vietoris-Rips & (from \citep{ballester2025expressivity}) & 0 (0\%)   & 0 (0\%)    & 0 (0\%)    & 3 (3\%)    & 4 (1\%)    \\
% \midrule
% NetLSD & \citep{tsitsulin2018netlsd,rozembereczki2020karateclub}& 60 (100.0\%)  & 50 (35.7\%) & 100 (100.0\%)  & 3 (3.0\%) & 213 (53.2\%)\\
% FEATHER & \citep{rozemberczki2020characteristic,rozembereczki2020karateclub} & 52 (86.6\%)  & 46 (32.9\%) & 5 (5.0\%)  & 0 (0.0\%) & 103 (31.0\%)\\
% %\midrule
% %Resistance Curvature Filtration &(from \citep{southern2023curvature})  & 56 (93.3\%)  & 50 (35.7\%) & 97 (97.0\%)  & 4 (4.0\%) & 207 (51.8\%)\\
% %\midrule
% %DivCurve & shortest path metric & 54 & 43 &  43& 3 & 143\\ 
% \midrule
% Div(G) & heat kernel distance & 60 (100.0\%) & 50 (35.7\%) &  92 (92.0\%) & 3 (3.0\%) & 205 (51.3\%)\\
% Div(G) &diffusion distance & 60 (100.0\%) & 49 (35.0\%) &  84 (84.0\%)  & 3 (3.0\%) & 196 (49.0\%)\\
% Div(G) &shortest path metric & 16 (26.7\%) & 13 (9.3\%) &  41 (41.0\%)& 6 (6.0\%)& 76 (19.0\%)\\ 
% \midrule
% DivCurve$(\mathcal{G}_{\{n-1, n\}})$ &heat kernel distance & 60 (100.0\%) & 65 (46.4\%) & 96 (96.0\%) &  3 (3.0\%) & 224 (51.3\%) \\ 
% DivCurve$(\mathcal{G}_{\{n-1, n\}})$ &diffusion distance & 60 (100.0\%) & 58 (41.4\%) & 94 (94.0\%) & 3 (3.0\%) & 215 (53.8\%)\\ 
% DivCurve$(\mathcal{G}_{\{n-1, n\}})$ &shortest path metric & 60 (100.0\%) & 48 (34.3\%) & 87 (87.0\%) & 8 (8.0\%) & 203 (50.8\%) \\ 

%  %& 0.90  & 0.5571 & 0.96   & 0.67   & 0.7375
% %All  & 60  & 140 & 100 & 100 & 400 \\
% %\\
% \bottomrule
% \end{tabular}}
% \label{tab:brec_main}
% \end{table}

\begin{table}[ht]

\caption{Number of pairs from the whole \texttt{BREC} dataset distinguished via structural diversity or diversity curves. Compared to representative results from \citep{wang2023empirical,southern2023curvature, ballester2025expressivity}.}
\centering
\begin{tabular}{llc}
\toprule
 Method & Details & All (400) \\
\midrule
%1 WL (from \citep{southern2023curvature}) & 207 (51.8\%)\\
%3 WL (from \citep{southern2023curvature}) & (51.8\%)\\
%\midrule
%Resistance Curvature (from \citep{southern2023curvature}) & 207 (51.8\%)\\
%OR Curvature (from \citep{southern2023curvature}) & 207 (51.8\%)\\
3 WL &(from \citep{wang2023empirical}) & 270 (67.5\%)\\
1 WL &(from \citep{southern2023curvature}) & 0 (0.0\%)\\
\midrule
% I2-GNN &(from \citep{wang2023empirical}) & 281 (70.2\%)\\
% KP-GNN &(from \citep{wang2023empirical}) & 275 (68.8\%)\\
% GSN &(from \citep{wang2023empirical}) & 254 (63.5\%)\\
% Graphormer &(from \citep{wang2023empirical}) & 79 (19.8\%)\\
% \midrule
% CurvPool &(from \citep{lachi2025expressive}) & 157 (39.3\%)\\
% XP &(from \citep{lachi2025expressive}) & 124 (31.0\%)\\
% EdgePool &(from \citep{lachi2025expressive}) & 23 (5.8\%)\\
% DiffPool &(from \citep{lachi2025expressive}) & 0 (0.0\%)\\
% \midrule
% PH Laplacian & (from \citep{ballester2025expressivity}) & 216 (54\%) \\
% PH Ollivier–Ricci Curvature & (from \citep{ballester2025expressivity}) & 208 (52\%) \\
% PH Forman–Ricci Curvature & (from \citep{ballester2025expressivity}) & 172 (43\%) \\
% PH Degree Filtration & (from \citep{ballester2025expressivity}) & 116 (29\%) \\
PH Vietoris-Rips & (from \citep{ballester2025expressivity}) & 84 (21\%) \\
%\midrule
%PH1 Laplacian & (from \citep{ballester2025expressivity}) & 160 (40\%) \\
%PH1 Ollivier–Ricci Curvature & (from \citep{ballester2025expressivity}) & 176 (44\%) \\
%PH1 Forman–Ricci Curvature & (from \citep{ballester2025expressivity}) & 132 (33\%) \\
%PH1 Degree Filtration & (from \citep{ballester2025expressivity}) & 12 (3\%) \\
%PH1 Vietoris-Rips & (from \citep{ballester2025expressivity}) & 4 (1\%) \\
\midrule
NetLSD & \citep{tsitsulin2018netlsd,rozembereczki2020karateclub} & 213 (53.2\%)\\
FEATHER & \citep{rozemberczki2020characteristic,rozembereczki2020karateclub} & 103 (31.0\%)\\
%\midrule
%Resistance Curvature Filtration &(from \citep{southern2023curvature}) & 207 (51.8\%)\\
%\midrule
%DivCurve & shortest path metric & 143\\
\midrule
Div(G) & heat kernel distance & 205 (51.3\%)\\
Div(G) &diffusion distance & 196 (49.0\%)\\
Div(G) &shortest path metric & 76 (19.0\%)\\
\midrule
DivCurve$(\mathcal{G}_{\{n-1, n\}})$ &heat kernel distance & 224 (51.3\%) \\
DivCurve$(\mathcal{G}_{\{n-1, n\}})$ &diffusion distance & 215 (53.8\%)\\
DivCurve$(\mathcal{G}_{\{n-1, n\}})$ &shortest path metric & 203 (50.8\%) \\

%All & 400 \\
%\\
\bottomrule
\end{tabular}
\label{tab:brec_main}
\end{table}

==> tables/generation.tex <==
\begin{minipage}[t]{0.43\textwidth}
\vspace{0pt} 
\captionof{table}{DiversityCurves distinguish between generated graphs.}
\centering
\label{tab:gen}
\resizebox{\linewidth}{!}{  
\begin{tabular}{llc}
\toprule
& Dataset  & Balanced Accuracy \\
\midrule
\multirow{2}{*}{Test / Generated}
 &Planar   & 0.660 $\pm$ 0.108 \\
 &SBM   & 0.628 $\pm$ 0.113 \\
 %&Optimal Generator   & 0.500 $\pm$ 0.000 \\
 \midrule
w/wo Hydrogens & QM9   & 0.988 $\pm$ 0.015 \\
 \multicolumn{2}{l}{ Planar / SBM / QM9} & 0.995 $\pm$ 0.007\\
\bottomrule
\end{tabular}}
\end{minipage}
\hspace{0.05\textwidth}
\begin{minipage}[t]{0.5\textwidth}
\vspace{0pt} % ensures top alignment
\centering
%\includegraphics[width=0.49\linewidth]{figures/single_cell/sc_curves_traj.png}
\includegraphics[width=1\linewidth]{figures/graph_generation/all.pdf}
\captionof{figure}{PCA plot of the DiversityCurves for all generated and test set graphs.}
\label{fig:gen_pca}
\end{minipage}
